Improved measurement of $C\!P$ violation in $B^{0}_{s} \!\to J/\psi \pi^{+}\pi^{-}$ decays

The time-dependent $C\!P$ asymmetry in $B^{0}_{s} \!\to J/\psi \pi^{+}\pi^{-}$ decays is measured using proton-proton collision data, corresponding to an integrated luminosity of $6\,\text{fb}^{-1}$, collected with the LHCb detector at a centre-of-mass energy of $13\,\text{TeV}$ during $\mbox{2015--2018}$. The $C\!P$-violating phase, $\phi_{s}$, the direct $C\!P$-violation parameter, $\left|\lambda\right|$, and the decay width of the heavy mass eigenstate in the $B^{0}_{s}$ system, $\Gamma_{\mathrm{ H}}$, are measured respectively to be $\phi_{s} = -0.077 \pm 0.034 \pm 0.007\,\text{rad}$, $\left|\lambda\right| = 0.993 \pm 0.026 \pm 0.007$ and $\Gamma_{\mathrm{ H}} = 0.610 \pm 0.002 \pm 0.004\,\text{ps}^{-1}$, where the first uncertainties are statistical and the second systematic. These results are consistent with previous measurements and the expectation based on the Standard Model. The combination with previous measurements in $B^{0}_{s} \!\to J/\psi \pi^{+}\pi^{-}$ decays using $7\,\text{TeV}$ and $8\,\text{TeV}$ proton-proton collision data yields $\phi_{s} = -0.046 \pm 0.031\,\text{rad}$, $\left|\lambda\right| = 0.975 \pm 0.024$ and $\Gamma_{\mathrm{ H}} = 0.610 \pm 0.004\,\text{ps}^{-1}$, while the combination including all other LHCb measurements gives $\phi_{s} = -0.041 \pm 0.017\,\text{rad}$.

==> LHCb/Authorship_LHCb-PAPER-20YY-nnn.tex <==
% ===============================================================================
% Purpose: example of authorlist for LHCb template
% Author:
% Created on: 2009-09-24
% ===============================================================================

%\documentclass[a4paper]{article}
%\setlength{\oddsidemargin}{0cm}
%\setlength{\evensidemargin}{0cm}
%\setlength{\textwidth}{16.5cm}
%\setlength{\parindent}{0cm}
%\begin{document}
\centerline{\large\normalfont\bfseries LHCb collaboration}
\begin{flushleft}
\small
%-- LHCb Authorlist, Example typesetting
%-- 
A.~N.~Other$^{1}$.\bigskip\newline{\it
\footnotesize
$ ^{1}$University of nowhere\\
}
%-- 
%-- 
\end{flushleft}
%\end{document}



